SCOReD: Student-Aware CoT Optimization for Recommendation Distillation

Chain-of-thought (CoT) distillation in the recommendation domain is a necessary precursor to RL training, but raw teacher traces are ill-suited to this task. Large teachers approach the recommendation task with unusually high reasoning uncertainty, repeatedly rechecking their answers without revising them; supervised fine-tuning on such traces produces verbose students that never revise their initial guess. Furthermore, due to the novelty of the recommendation domain, the teacher's reasoning traces are highly out-of-distribution for the small student LLM. We propose Student-Aware CoT Optimization for Recommendation Distillation (SCOReD), a CoT optimization framework tailored to recommendation that first parses each teacher trace into typed segments and uses the student LLM's attention to score the importance of each segment. Then SCOReD dynamically selects a per-segment edit (KEEP / REWRITE / FUSE / PRUNE) based on the output length and comparative log probability lift of the answer given the edit as per the student. Therefore, SCOReD prunes redundant sections of the reasoning trace while preserving information-dense sections and adapts raw teacher traces to the student's output distribution. Training on SCOReD-optimized CoTs provides a cleaner learning signal to the student model and improves over baseline SFT by 1.56% NDCG and 1.9% Recall@5, while reducing reasoning length by 27.3%.

==> assets/old_method_1.tex <==

\subsection{LLM-Based CoT Segmentation}
\label{sec:segmentation}

We first generate K reasoning traces from our teacher LLM Google Gemma-4-26B with the following prompt:
\begin{promptbox}{Recommendation Prompt}
You are a recommendation assistant. You will receive a user's purchase history and a numbered list of candidate items. Your task is to rank all candidates from most to least likely to match the user's preferences, where preference is inferred from thematic, categorical, and ingredient/style similarity to past purchases.

Output format: Return only a Python-style list containing every candidate number exactly once, ordered from most to least preferred. Example for 10 candidates: [3, 6, 7, 2, 4, 9, 10, 5, 1, 8]. Do not include explanations, commentary, or any text outside the list in the final answer.
\end{promptbox}

This is similar to rejection sampling used by \citep{liang2026gr2}, but instead of an exact match with the ground truth, we take select the CoT that corresponds to the highest NDCG score, tie-breaking on shorter CoT length. 


Notably, the recommendation prompt imposes no formatting constraints on the teacher LLM's reasoning chain, only on the output. \citet{yuehhan2026reasoningmodelsstrugglecontrol} has shown that reasoning LLMs can control their CoT only 2.7\% of the time. As such, we formulate structured reasoning as a post-hoc extraction step using another LLM. 


After generating the CoTs with the teacher LLM, we use Gemma-4-26B to parse the trace into a sequence of segments $S_1, \dots, S_n$, each labeled with one of six types: Purchase History Review, User Interest Modeling, Candidate Analysis, Intermediate Ranking, Verification, and Final Ranking.

\begin{promptbox}{LLM Segmenter Prompt}
You are an expert data annotator. Your task is to segment a reranking reasoning chain into contiguous blocks belonging to one of the following stages:
H: Purchase History Analysis (summarizing or categorizing past purchases)
P: User Preference / Theme Modeling (inferring categories, brands, ingredients, benefits, or use cases from history)
C: Candidate Analysis (describing candidate items and their relevance before constructing the ranking)
R: Ranking Construction / Tiering (building tiers, assigning rank positions, or forming a preliminary ordered list)
V: Verification / Pairwise Comparison / Self-Correction (checking close calls, comparing candidates, expressing doubt, or revising the order)
F: Final Ranking (the final conclusion, final order, or final ranked list inside the reasoning chain)

Common reranking patterns include candidate summaries, high/mid/low tiers, pairwise comparisons like 'candidate 5 vs candidate 6', repeated 'Wait' checks, and one or more final ordered lists.

CRITICAL RULES:
1. You will be given the reasoning chain with line numbers.
2. Output your response STRICTLY as a JSON array of objects. Each object must have 'stage' (string, one of H, P, C, R, V, F), 'start_line' (int), and 'end_line' (int).
3. The segments must cover all lines from {first_line} to {final_line} continuously, with no gaps or overlaps.
4. Segment at HIGH GRANULARITY. Break down long blocks when the reasoning shifts between history, preferences, candidate analysis, tiering, verification, and final ranking.
5. Do not label every ordered list as F. Use F only for final conclusions or final ranking statements; use R for intermediate tiering and draft rankings.
6. Output ONLY the valid JSON array. Do not include markdown formatting like ```json.
\end{promptbox}


Table~\ref{tab:stage-stats} summarizes segment-level statistics over $289{,}541$ annotated blocks.
Verification (\textbf{V}) and ranking (\textbf{R}) dominate the segmentation: together they account for ${\approx}63\%$ of all segments.
Final-ranking blocks (\textbf{F}) are shorter on average, consistent with concise conclusion statements.

\begin{table}[t]
\centering
\caption{Segmentation stage distribution (segment-level counts).}
\label{tab:stage-stats}
\begin{tabular}{lrrr}
\toprule
Stage & Share & Avg.\ chars/seg & Role \\
\midrule
V (verification)      & 33.9\% & 418 & Pairwise checks, doubts, revisions \\
R (ranking)           & 29.4\% & 367 & Tiering, draft orderings \\
C (candidate analysis)& 15.3\% & 459 & Per-candidate relevance \\
F (final ranking)     &  7.3\% & 120 & Final ordered conclusions \\
P (preference)        &  7.1\% & 169 & Theme / preference inference \\
H (purchase history)  &  7.0\% & 268 & History summarization \\
\bottomrule
\end{tabular}
\end{table}

At the \emph{trajectory} level (one rollout per row), samples contain a median of $23$ segments ($\mu{=}25.5$, $\sigma{=}10.6$) and $6$ distinct stage labels in $91.9\%$ of cases.
Stages \textbf{C}, \textbf{R}, and \textbf{V} appear in every segmented rollout; \textbf{F} is absent in $6.6\%$ of samples.

\subsection{Stage transition structure}

Adjacent-segment transitions ($278{,}191$ total; stitching merges consecutive same-stage blocks, so self-transitions are $0$) reveal a pronounced \textbf{R}$\leftrightarrow$\textbf{V} loop.
The two most common edges are \textbf{R}$\to$\textbf{V} ($25.3\%$) and \textbf{V}$\to$\textbf{R} ($18.8\%$), followed by \textbf{C}$\to$\textbf{R} and cross-links from \textbf{V} back to \textbf{C}.
The canonical opening is \textbf{H}$\to$\textbf{P}$\to$\textbf{C}$\to$\textbf{R} (82.4\% of rollouts).

Table~\ref{tab:transition-counts} gives raw adjacent-segment transition counts $N_{ij}$ (row~$i$, column~$j$).
Cell shading is proportional to count (deeper blue = more transitions; white = zero or diagonal placeholder).

\begin{table}[t]
\centering
\caption{Adjacent stage transition counts $N_{ij}$ (blue heatmap; max cell $=70{,}414$).}
\label{tab:transition-counts}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l|rrrrrr}
\toprule
From $\backslash$ To & H & P & C & R & V & F \\
\midrule
H & \cellcolor{white}{0} & \cellcolor{blue!17}{12{,}130} & \cellcolor{blue!8}{4{,}204} & \cellcolor{blue!8}{1{,}343} & \cellcolor{blue!8}{2{,}620} & \cellcolor{blue!8}{104} \\
P & \cellcolor{blue!8}{126} & \cellcolor{white}{0} & \cellcolor{blue!20}{13{,}943} & \cellcolor{blue!8}{4{,}343} & \cellcolor{blue!8}{1{,}736} & \cellcolor{blue!8}{321} \\
C & \cellcolor{blue!8}{912} & \cellcolor{blue!8}{2{,}475} & \cellcolor{white}{0} & \cellcolor{blue!34}{23{,}749} & \cellcolor{blue!22}{15{,}436} & \cellcolor{blue!8}{1{,}558} \\
R & \cellcolor{blue!8}{2{,}390} & \cellcolor{blue!8}{1{,}345} & \cellcolor{blue!11}{7{,}862} & \cellcolor{white}{0} & \cellcolor{blue!100}{\textcolor{white}{70{,}414}} & \cellcolor{blue!8}{2{,}337} \\
V & \cellcolor{blue!8}{4{,}768} & \cellcolor{blue!8}{4{,}415} & \cellcolor{blue!25}{17{,}433} & \cellcolor{blue!74}{\textcolor{white}{52{,}407}} & \cellcolor{white}{0} & \cellcolor{blue!24}{16{,}687} \\
F & \cellcolor{blue!8}{880} & \cellcolor{blue!8}{95} & \cellcolor{blue!8}{849} & \cellcolor{blue!8}{3{,}233} & \cellcolor{blue!11}{8{,}076} & \cellcolor{white}{0} \\
\bottomrule
\end{tabular}
\end{table}


After segmentation, we discover a few dominant patterns. 

1. The teacher's CoT always beings with H, P, C, R. The teacher first summarizes user's purchases in P, categorizing them and noting dominant patterns. Based on these, the teacher determines the interests of the user at segment P. It then reviews the candidates (C), matching them to the purchases and making an initial ranking R. From there, the teacher undertakes serveral refinement loops, characterized by R $\rightarrow$ V $\rightarrow$ R or R $\rightarrow$ V $\rightarrow$ C $\rightarrow$ R transitions. On average, the teacher's raw CoT contains $8.65\pm4.17$ V stages, highlighting the high uncertainty of the even a capable teacher in the recommendation domain.

Surprisingly, although raw CoTs contain 8.65 V steps on average, only 47.15\% traces have a final ranking that is different from the initial ranking. This means that 92.89\% of refinement loops do not change the ranking suggestion. Therefore, training the student on raw traces does not teach backtracking or refinement, rather to reinforce the initial ranking suggestion while ballooning CoT length.

\paragraph{Is The Number of Refinement Attempts Predictable?} We investigate whether lexical features of the prompt can predict the number of refinements attempted by the teacher. For example, does a long purchase history lead the teacher to undertake more refinement loops? We find that the prompt length, length of purchase history, or the textual overlap between purchased items and candidate items do not predict the number of refinement attempts (-0.08, -0.05 and -0.11 pearson against number of V stages). This shows that the number of refinement attempts by the teacher is highly context dependent and cannot be predicted from simple lexical features, highlighting the difficulty of the recommendation domain for LLMs.



